$\pi^0$ and $\eta$ meson production in proton-proton collisions at $\sqrt{s}=8$ TeV

An invariant differential cross section measurement of inclusive $\pi^{0}$ and $\eta$ meson production at mid-rapidity in pp collisions at $\sqrt{s}=8$ TeV was carried out by the ALICE experiment at the LHC. The spectra of $\pi^{0}$ and $\eta$ mesons were measured in transverse momentum ranges of $0.3<p_{\rm T}<35$ GeV/$c$ and $0.5<p_{\rm T}<35$ GeV/$c$, respectively. Next-to-leading order perturbative QCD calculations using fragmentation functions DSS14 for the $\pi^{0}$ and AESSS for the $\eta$ overestimate the cross sections of both neutral mesons, although such calculations agree with the measured $\eta/\pi^{0}$ ratio within uncertainties. The results were also compared with PYTHIA~8.2 predictions for which the Monash~2013 tune yields the best agreement with the measured neutral meson spectra. The measurements confirm a universal behavior of the $\eta/\pi^{0}$ ratio seen for NA27, PHENIX and ALICE data for pp collisions from $\sqrt{s}=27.5$ GeV to $\sqrt{s}=8$ TeV within experimental uncertainties. A relation between the $\pi^{0}$ and $\eta$ production cross sections for pp collisions at $\sqrt{s}=8$ TeV is given by $m_{\rm T}$ scaling for $p_{\rm T}>3.5$ GeV/$c$. However, a deviation from this empirical scaling rule is observed for transverse momenta below $p_{\rm T}<3.5$ GeV/$c$ in the $\eta/\pi^0$ ratio with a significance of $6.2\sigma$.

==> Bibliography.tex <==
\begin{thebibliography}{99}
\bibitem{PublicNote8TeV}
  \textcolor{red}{Public note of 8 TeV analysis}
\bibitem{LHC}
  Lyndon Evans and Philip Bryant, "LHC Machine",  $JINST{\rm 3}$ (2008) S08001.
\bibitem{QCD}
  David J. Gross and Frank Wilczek, "Asymptotically Free Gauge Theories. I", Phys. Rev. D 8, 3633 (1973).
\bibitem{ALICE}
  ALICE Collaboration, K. Aamodtet al., "The ALICE experiment at the CERN LHC" $JINST{\rm 3}$ (2008) S08002.
\bibitem{PHOS}
  ALICE Collaboration, G. Dellacasa et al., "LICE technical design report of the photon spectrometer (PHOS)," $CERN$-$LHCC$-$99$-$04$ (1999).
\bibitem{EMCal}
  ALICE Collaboration, P. Cortese et al., "ALICE electromagnetic calorimeter technical design 414 report,".
\bibitem{ITS}
  ALICE Collaboration, K. Aamodt et al., "Alignment of the ALICE Inner Tracking System with cosmic-ray tracks," $JINST{\rm 5}$ (2010) P03003.
\bibitem{TPC}
  J. Alme, Y. Andres, H. Appelshauser, S. Bablok, N. Bialas, et al., "The ALICE TPC, a large 3-dimensional tracking device with fast readout for ultra-high multiplicity events," $Nucl.Instrum.Meth.$ A622 (2010) 316–367.
\bibitem{V0}
  ALICE Collaboration, P. Cortese et al., "ALICE technical design report on forward detectors: FMD, T0 and V0," $CERN$-$LHCC$-$2004$-$025$ (2004).
\bibitem{DeFlorian2015}
  D. Florian, R. Sassot, M. Epele, R. J. Hernández-Pinto and M. Stratmann, "Parton-to-Pion Fragmentation Reloaded" Phys.Rev. D91 (2015).
\bibitem{MB}
  ALICE Collaboration, B. Abelev et al., "Measurement of inelastic, single- and double-diffraction cross sections in proton–proton collisions at the LHC with ALICE," $Eur.$ $Phys.$ $J.$ C73 no. 6, (2013) 2456.
\bibitem{ALICE_Performance}
  ALICE Collaboration, "Performance of the ALICE Experiment at the CERN LHC", Int. J. Mod. Phys. A 29 (2014) 1430044.
\bibitem{PHOSTrigger}
  D. Wang et al., "Level-0 trigger algorithms for the ALICE PHOS detector," $Nucl.Instrum.Meth.$ A629 (2011) 80-86.
\bibitem{EMCalTrigger}
  ALICE EMCal Collaboration, U. Abeysekara et al., "ALICE EMCal Physics Performance Report", 1008.0413, arXiv:1008.0413.
\bibitem{vdMScan}
  Van der Meer, "Calibration of the Effective Beam Height in the ISR", Internal CERN report, ISR-PO/68-31 (1968).
\bibitem{vdMScan8TeV}
  \textcolor{red}{van der Meer scan note for 8 TeV}
\bibitem{PDG}
  Particle Data Group Collaboration, K. A. Olive et al., "Review of Particle Physics," $Chin.$ $Phys.$ C38 (2014) 090001.
\bibitem{ArmenterosPodolanski}
  J. Podolanski and R. Armenteros, Phil. Mag. 45, (1954) 13.
\bibitem{CrystalBall}
   F. James and M. Roos.  Minuit - a system for function minimization and analysis of the parameter  errors  and  correlations. Computer Physics Communications, 10(6):343-367, 1975.
\bibitem{PYTHIA82}
  T. Sjostrand, S. Mrenna, and P. Skands, "Brief Introduction to PYTHIA 8.1," Comput. Phys. Comm. 178 (2008).
\bibitem{Geant3}
  R. Brun, F. Bruyant, M. Maire, A. McPherson, and P. Zanarini, "GEANT3" Tech. Rep. CERN-DD-EE-84-1, CERN, 1987.
\bibitem{NeutralPion7000GeV}
  ALICE Collaboration, B. B. Abelev et al., "Neutral pion and $\eta$ meson production in proton-proton collisions at $\sqrt{s}$ = 0.9 TeV and $\sqrt{s}$ = 7 TeV," Phys. Lett. B717 (2012) 162–172. 
\bibitem{NeutralPion2760GeV}
  ALICE Collaboration, B. B. Abelev et al., "Neutral pion production at midrapidity in pp and Pb-Pb collisions at $\sqrt{s_{NN}}$ = 2.76 TeV," $Eur. Phys. J.$ C74 no. 10, (2014) 3108.
\bibitem{TwoComponentModel}
  A. R. Alexander Bylinkin, Nadezda Chernyavskaya, "Predictions on the transverse momentum spectra for charged particle production at lhc-energies from a two component model," $Eur. Phys. J.$ C(2015) 75:166.
\bibitem{MSTW}
  R.S. Thorne, A.D. Martin, W.J. Stirling and G. Watt, "Status of MRST/MSTW PDF sets", arXiv:0907.2387.
\bibitem{DSS14}
  D. Florian, R. Sassot, M. Epele, R. J. Hernández-Pinto and M. Stratmann, ``Parton-to-Pion Fragmentation Reloaded'' Phys. Rev. D91 (2015).
\bibitem{CTEQ6M5}
  J. Pumplin, D. Stump, J. Huston, H. Lai, P. M. Nadolsky, et al., "New generation of parton distributions with uncertainties from global QCD analysis," $JHEP$ 0207 (2002) 012.
\bibitem{AESSS}
   C. A. Aidala, F. Ellinghaus, R. Sassot, J. P. Seele and M. Stratmann, "Global Analysis of Fragmentation Functions for Eta Mesons," Phys. Rev. D83 034002, 2011.
\bibitem{Monash2013}
  P. Skands, S. Carrazza and J. Rojo, "Tuning PYTHIA 8.1: the Monash 2013 tune," $Eur. Phys. J.$ C(2014) 74:30124.
\bibitem{Tune4C}
  R. Corke and T. Sjostrand, "Interleaved parton showers and tuning prospects", $JHEP$ 03 (2011) 032.
\bibitem{RHIC510GeV}
  PHENIX Collaboration, A. Adare et al., "Inclusive cross section and double-helicity asymmetry for $\pi^{0}$ production at midrapidity in $p$+$p$ collisions at $\sqrt{s}=510$ GeV", Phys. Rev. D 93, 011501 (2016).
\end{thebibliography}

